Parameter-Efficient Conversational Recommender System as a Language Processing Task

Conversational recommender systems (CRS) aim to recommend relevant items to users by eliciting user preference through natural language conversation. Prior work often utilizes external knowledge graphs for items' semantic information, a language model for dialogue generation, and a recommendation module for ranking relevant items. This combination of multiple components suffers from a cumbersome training process, and leads to semantic misalignment issues between dialogue generation and item recommendation. In this paper, we represent items in natural language and formulate CRS as a natural language processing task. Accordingly, we leverage the power of pre-trained language models to encode items, understand user intent via conversation, perform item recommendation through semantic matching, and generate dialogues. As a unified model, our PECRS (Parameter-Efficient CRS), can be optimized in a single stage, without relying on non-textual metadata such as a knowledge graph. Experiments on two benchmark CRS datasets, ReDial and INSPIRED, demonstrate the effectiveness of PECRS on recommendation and conversation. Our code is available at: https://github.com/Ravoxsg/efficient_unified_crs.

==> Sections/architecture.tex <==
%In this section, we describe our approach to the CRS task, named \textbf{UPCRS} for \textbf{U}nified \textbf{P}arameter-efficient \textbf{C}onversational \textbf{R}ecommender \textbf{S}ystem.

\paragraph{Overview.}
Formally, we denote the $\bm{I}=\{\bm{I}_{1}, \ldots, \bm{I}_{M}\}$ as item set, made of $M$ items. Meanwhile, the CRS dataset contains $N$ dialogue contexts, noted as $\bm{C}=\{\bm{C}_{1}, \ldots, \bm{C}_{N}\}$, each coupled with a response, which set is denoted as $\bm{Y}=\{\bm{Y}_{1}, \ldots, \bm{Y}_{N}\}$. The model task is to predict the correct $\bm{I}_{j}$ and exact response $\bm{Y}_{i}$ associated to context $\bm{C}_{i}$. We use a single decoder-only language model with dedicated prediction heads to support both tasks. The overall architecture of the proposed \textbf{U}nified \textbf{P}arameter-efficient \textbf{C}onversational \textbf{R}ecommender \textbf{S}ystem (UPCRS) is shown in \Cref{fig:2}. 
\red{TODO}
Next, we present each module of UPCRS in detail.

\paragraph{Recommendation.}
Following high-performing approaches in CRS~\cite{unicrs, mese}, we model the recommendation prediction as maximizing the similarity between a representation of the dialogue context, and a representation of the item to predict. Each item $\bm{I}_{j}$ is encoded as a string containing the item name followed by metadata, for a total of $m_{j}$ tokens: $\bm{I}_{j}=s_{j,1} \ldots s_{j,m_{j}}$. Similarly, we represent the i-th context as a string of $n_{i}$ tokens: $\bm{C}_{i}=c_{i,1} \ldots c_{i,n_{i}}$. In a generic case, let us now denote by $\gamma$ the parameters of the model encoding each item and by $\omega$ the parameters of the dialogue response decoder. The probability that the CRS system recommends item $\bm{I}_{j}$ to dialogue context $\bm{C}_{i}$ is:

\begin{equation}
    p_{i,j} = \frac{e^{\gamma(\bm{I}_{j}) \bm{\cdot} \omega(\bm{C}_{i})}}{\sum_{\substack{k=1}}^{M} e^{\gamma(\bm{I}_{k}) \bm{\cdot} \omega(\bm{C}_{i})}}
\end{equation}

Where $\gamma(\bm{I}_{j})$ and $\omega(\bm{C}_{i})$ are \emph{pooled} outputs, and $\bm{\cdot}$ can be any high-dimensional space distance or similarity function (e.g., Euclidian distance). 

In this paper, instead of using separate neural networks, we parameterize the representation of items and of dialog contexts by the \emph{same} model. More specifically, let us note $\theta$ the parameters of a decoder-only neural network (e.g., GPT-2). $\theta(\bm{X})$ represents the \emph{unpooled}, last hidden layer output from model $\theta$ on input tokens vector $\bm{X}$. Because of causal self-attention, we can use the last token to represent the whole dialogue, as it attends to all previous tokens:

\begin{equation}
    \omega(\bm{C}_{i}) = h_{dial}(\theta(C_{i,n_{i}}))
\end{equation}

Where $h_{dial}$ is a projection head. Such a process cannot naturally be applied to reducing the items representation, since the metadata text does not follow a causal order. Therefore, we use a learnable pooling layer $\rho$, followed by an items head $h_{item}$, to represent each item:

\begin{equation}
    \gamma(\bm{I}_{j}) = h_{item}(\rho(\theta(\bm{I}_{j})))
\end{equation}

The recommendation probability becomes:

\begin{equation}
\label{eq:4}
    p_{i,j} = \frac{e^{h_{item}(\rho(\theta(\bm{I}_{j}))) \bm{\cdot} h_{dial}(\theta(C_{i,n_{i}}))}}{\sum_{\substack{k=1}}^{M} e^{h_{item}(\rho(\theta(\bm{I}_{k}))) \bm{\cdot} h_{dial}(\theta(C_{i,n_{i}}))}}
\end{equation}

In practice, we have $|\rho|,|h_{dial}|,|h_{item}| << |\theta|$, so our approach makes a better use of the system parameters. A key element in UPCRS is a \emph{\textbf{stop-gradient}} operator when using the decoder to encode items. Indeed, since the number of items can be large, and items need to be sequentially encoded before encoding the dialogue context, the backward pass becomes too computationally intensive. To bypass this issue, we stop the gradient related to items encoding (noted as $\theta_{\bm{sg}}$), which drastically reduces compute time and memory usage. The model is able to pull from the knowledge contained in $\theta$ and adjust items representations through $h_{item}$. 

The final recommendation probability is:

\begin{equation}
    p_{i,j} = \frac{e^{h_{item}(\rho(\theta_{\bm{sg}}(\bm{I}_{j}))) \bm{\cdot} h_{dial}(\theta(C_{i,n_{i}}))}}{\sum_{\substack{k=1}}^{M} e^{h_{item}(\rho(\theta_{\bm{sg}}(\bm{I}_{k}))) \bm{\cdot} h_{dial}(\theta(C_{i,n_{i}}))}}
\end{equation}

\begin{figure*}
    \includegraphics[width=\textwidth]{emnlp2023-latex/Images/architecture.png}
    \caption{Architecture of UPCRS. Light blue cells correspond to learnable model parameters.}
    \label{fig:2}
\end{figure*}

\paragraph{Response Generation.}
The backbone model $\theta$ is a decoder language model, which is naturally suited for response generation. For the i-th data point, ground truth response $\bm{Y}_{i}$ is broken down into its tokens: $\bm{Y}_{i}=y_{i,1} \ldots y_{i,t_{i}}$. Then, the probability assigned by $\theta$ to predict the correct k-th ground truth token (where $1 \leq k \leq t_{i}$) can be written as:
\begin{equation}
p(y_{i,k} | \bm{C}_{i}, y_{i,1} \ldots y_{i,k-1} ; \theta)
\end{equation}

\paragraph{Parameter-efficient Learning.}
Since the backbone decoder LM is pre-trained with auto-regressive language modeling, it is naturally suited for dialogue response prediction. Fine-tuning this model for very different tasks such as items recall might lead to catastrophic forgetting. To prevent this issue, we keep the decoder frozen, and leverage the recently introduced LoRA parameter-efficiency technique \citep{lora}, which consists of low-rank weight matrices in parallel of the standard Transformer blocks. Only fine-tuning LoRA blocks can surpass fine-tuning of all parameters, and was successfully leveraged for instruction-tuning of very large LMs \citep{llmadapter}. On top of LoRA layers, we also update the embeddings of new special tokens marking recommendation \citep{mese}, the item pooling and head, and MLP for recall and re-ranking projections, which maintains a very small (under 5\%) fraction of learned parameters.



==> Sections/training.tex <==
To train the system, we follow the multi-tasking framework in MESE \citep{mese}. 

\paragraph{Recommendation.}
First, a cross-entropy loss is minimized to enforce the model to assign high probability to the correct item assigned to each dialogue context. Noting $l_{i}$ the index of the ground-truth item associated with context $\bm{C}_{i}$, then the recall loss is expressed as:

\begin{equation}
    \mathcal{L}_{recall} = -\log(p_{i,l_{i}})
\end{equation}

Next, the sampled items are re-ranked, for a finer-grained retrieval prediction. Each item $\bm{I}_{j}$ is assigned the following relevance score with regards to context $C_{i}$:

\begin{equation}
\label{eq:7}
    r_{i,j} = \frac{e^{h_{item}(\rho(\theta([\bm{C}_{i},\bm{I}_{j}])))}}{\sum_{\substack{k=1}}^{M} e^{h_{item}(\rho(\theta([\bm{C}_{i},\bm{I}_{k}])))}}
\end{equation}

Where $[\bm{C}_{i},\bm{I}_{k}]$ is the concatenation between context $C_{i}$ and candidate item $I_{k}$. In other words, the re-ranking score represents the probability mass assigned to the item when conditioned on the dialogue context. The re-ranking loss is a cross-entropy maximizing the probability assigned to the ground-truth item $\bm{I}_{l_{i}}$:

\begin{equation}
    \mathcal{L}_{rerank} = -\log(r_{i,l_{i}})
\end{equation}

\paragraph{Conversation.}
Lastly, the model is also trained to generate the response with the standard cross-entropy:

\vspace{-1.0em}
\begin{equation}
    \mathcal{L}_{gen} = -\sum_{\substack{k=1}}^{k=t_{i}} \log(p(y_{i,k} | \bm{C}_{i}, y_{i,1} \ldots y_{i,k-1} ; \theta))
\end{equation}

\paragraph{Multi-task training.}
The final loss is a linear combination of these three losses:

\vspace{-1.0em}
\begin{equation}
    \mathcal{L} = \alpha.\mathcal{L}_{recall} + \beta.\mathcal{L}_{rerank} + \gamma.\mathcal{L}_{gen}
\end{equation}

Where $\alpha$, $\beta$, $\gamma$ are fixed coefficients. 


\paragraph{Negative Sampling.}
We share the negative sampled items used for the computation of $\mathcal{L}_{recall}$ and $\mathcal{L}_{rerank}$. We also share negatives \emph{across batch elements}. This way, only one sampling process occurs for each batch: $M$ items are sampled, ensuring that none of them is a positive for any of the dialogue contexts in the batch. These negative items and the positive are concatenated and encoded following \Cref{sec:3}. During inference, we first encode the entire items bank. The $M$ items receiving the highest probability from \Cref{eq:4} are then passed through re-ranking, and the item with the highest final score from \Cref{eq:7} is taken as the system output recommendation. We decouple the value of $M$ between training and inference, such that $M_{training} < M_{inference}$. As we show in \Cref{subsec:5.3}, $M$ yields a trade-off between computation and recommendation performance. 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Optimization}

%We experiment with three different backbone decoders $\theta$ of varying size: GPT-2 small, GPT-2 medium, and GPT-2 large \citep{gpt2} referred to as \textbf{UPCRS-small}, \textbf{UPCRS-medium} and \textbf{UPCRS-large} respectively. As distance function $\bm{\cdot}$, we use the \emph{angular} distance between item embeddings and dialog representations. We sample $M_{train}=150$ candidate items for training, and $M_{inference}=700$ for inference. We train the model for 10 epochs, validating every epoch, using an effective batch size of 8. We linearly warmup the learning rate throughout the first epoch to a peak value of $0.00003$ for small and medium models, $0.00001$ for the large one, and train with the AdamW optimizer \citep{adamw}. During training, we balance losses with $\alpha=0.15$, $\beta=0.85$, and $\gamma=1.0$. We cap the length of dialogue context at 256 tokens and the length of generated responses at 64 tokens. We train the small and base models on a single Nvidia Tesla V100 GPU, and the large version on 2 V100.

==> Tables/8_m.tex <==

\begin{table}[]
\resizebox{\columnwidth}{!}{  
\begin{tabular}{llcccccc}

\toprule

$M_{training}$
& $M_{inference}$ 
& \textbf{\begin{tabular}[c]{@{}c@{}}Training\\ time/batch (s)\end{tabular}} 
& \textbf{\begin{tabular}[c]{@{}c@{}}Inference\\ time/batch (s)\end{tabular}} 
& \textbf{R@1} 
& \textbf{R@10} 
& \textbf{R@50} 
& \textbf{Unique} \\

\midrule 

\multirow{3}{*}{50}          
& 300        & & & & & & \\
& 500        & & & & & & \\
& 700        & & & & & & \\
           
\hdashline 

\multirow{3}{*}{100}         
& 300        & & & & & & \\
& 500        & & & & & & \\
& 700        & & & & & & \\
           
\hdashline 

\multirow{3}{*}{150}         
& 300        & & & & & & \\
& 500        & & & & & & \\
& 700        & & & 4.7 & 20.8 & 40.5 & 463 \\
           
\toprule 
           
\end{tabular}
}
\caption{Impact of the number of sampled item candidates, during training ($M_{\text{train}}$) and inference ($M_{\text{inference}}$). Results are shown for PECRS-small on the ReDial test set, in the recommendation task.}
\label{m}
\end{table}
